CRAB: Codebook Rebalancing for Bias Mitigation in Generative Recommendation

Generative recommendation (GeneRec) has introduced a new paradigm that represents items as discrete semantic tokens and predicts items in a generative manner. Despite its strong performance across multiple recommendation tasks, existing GeneRec approaches still suffer from severe popularity bias and may even exacerbate it. In this work, we conduct a comprehensive empirical analysis to uncover the root causes of this phenomenon, yielding two core insights: 1) imbalanced tokenization inherits and can further amplify popularity bias from historical item interactions; 2) current training procedures disproportionately favor popular tokens while neglecting semantic relationships among tokens, thereby intensifying popularity bias. Building on these insights, we propose CRAB, a post-hoc debiasing strategy for GeneRec that alleviates popularity bias by mitigating frequency imbalance among semantic tokens. Specifically, given a well-trained model, we first rebalance the codebook by splitting over-popular tokens while preserving their hierarchical semantic structure. Based on the adjusted codebook, we further introduce a tree-structured regularizer to enhance semantic consistency, encouraging more informative representations for unpopular tokens during training. Experiments on real-world datasets demonstrate that CRAB significantly improves recommendation performance by effectively alleviating popularity bias.

==> Attack_Result.tex <==
\begin{table*}[ht!]
.\caption{\label{tab:Result80}
$HR@10\times100$ for different attacks with $80\%$ training data (left) and $30\%$ training data (right) on two datasets.
}

%\vspace{-2mm}
\scalebox{0.75}{
\centering
\begin{tabular}{lll|cccc|}
\cline{4-7}
& & & \multicolumn{4}{c|}{{\bf Percentage of Cotrolled Users}}
\\
\hline
 \multicolumn{1}{|l|}{\bf Dataset} & \multicolumn{1}{l}{\thead{Recommendation\\Model}} & \multicolumn{1}{|l|}{\thead{Attack\\Method}} & \multicolumn{1}{c|}{\thead{$0.5\%$}} & \multicolumn{1}{c|}{\thead{$1\%$}} & \multicolumn{1}{c|}{\thead{$3\%$}} & \multicolumn{1}{c|}{\thead{$5\%$}}
\\
\hline
\multicolumn{1}{|l|}{\multirow{8}{*}{\em MovieLens}} & 
\multicolumn{1}{l}{\multirow{4}{*}{NCF}} & 
% \multicolumn{1}{|l|}{{\sc Random}} &
% \multicolumn{1}{c|}{$8.32 (\pm 0.63)$} & 
% \multicolumn{1}{c|}{$5.00 (\pm 1.20)$} &
% \multicolumn{1}{c|}{$8.70 (\pm 0.47)$} & 
% \multicolumn{1}{c|}{$5.23 (\pm 0.85)$} &
% \multicolumn{1}{c|}{$9.10 (\pm 0.49)$} & 
% \multicolumn{1}{c|}{$5.00 (\pm 1.20)$}
% \\
% \cline{3-9}
% \multicolumn{1}{|l|}{} &
% &
\multicolumn{1}{|l|}{{DL-Attack}} & 
\multicolumn{1}{c|}{$0.34$} & 
\multicolumn{1}{c|}{$0.39$} &
 \multicolumn{1}{c|}{$0.72$} & 
\multicolumn{1}{c|}{$0.82$} 
\\
\cline{3-7}
\multicolumn{1}{|l|}{} &
&
\multicolumn{1}{|l|}{{RAPU-R}} & 
\multicolumn{1}{c|}{$0.32$} &
\multicolumn{1}{c|}{$0.38$} &
\multicolumn{1}{c|}{$0.79$} & 
\multicolumn{1}{c|}{$0.86$} 
\\
\cline{3-7}
 \multicolumn{1}{|l|}{} &
 &
 \multicolumn{1}{|l|}{H-CARS} &
\multicolumn{1}{c|}{$\bf{0.37}$} & 
\multicolumn{1}{c|}{$\bf{0.42}$} &
\multicolumn{1}{c|}{$\bf{0.82}$} & 
\multicolumn{1}{c|}{$\bf{0.91}$} 
\\
\cline{3-7}
 \multicolumn{1}{|l|}{} &
 &
 \multicolumn{1}{|l|}{Bandwagon} &
\multicolumn{1}{c|}{$0.09$} & 
\multicolumn{1}{c|}{$0.11$} &
\multicolumn{1}{c|}{$0.16$} & 
\multicolumn{1}{c|}{$0.26$}



\\
\cline{2-7}
\multicolumn{1}{|l|}{} & 
\multicolumn{1}{l}{\multirow{4}{*}{RCF}} & 
% \multicolumn{1}{|l|}{{\sc Random}} &
% \multicolumn{1}{c|}{${\bf5.81} (\pm 0.38)$} & \multicolumn{1}{c|}{${\bf4.59} (\pm 0.33)$} & 
% \multicolumn{1}{c|}{$7.52 (\pm 0.47)$} &
% \multicolumn{1}{c|}{$5.17 (\pm 1.09)$} &
% \multicolumn{1}{c|}{$8.19 (\pm 0.21)$} & 
% \multicolumn{1}{c|}{$8.20 (\pm 1.60)$} 
% \\
% \cline{3-9}
% \multicolumn{1}{|l|}{} &
% &
\multicolumn{1}{|l|}{{DL-Attack}} & 
 \multicolumn{1}{c|}{$\bf{0.25}$} &
\multicolumn{1}{c|}{$\bf{0.29}$} &
 \multicolumn{1}{c|}{$0.63$} & 
\multicolumn{1}{c|}{$0.71$} 

\\
\cline{3-7}
\multicolumn{1}{|l|}{} &
&
\multicolumn{1}{|l|}{{RAPU-R}} & 
 \multicolumn{1}{c|}{$0.23$} & 
\multicolumn{1}{c|}{$0.28$} &
\multicolumn{1}{c|}{$0.66$} & 
\multicolumn{1}{c|}{$0.73$} 

\\
\cline{3-7}
\multicolumn{1}{|l|}{} &
&
\multicolumn{1}{|l|}{H-CARS} &
 \multicolumn{1}{c|}{$0.24$} & 
\multicolumn{1}{c|}{$\bf{0.29}$} & 
\multicolumn{1}{c|}{$\bf{0.68}$} & 
\multicolumn{1}{c|}{$\bf{0.76}$} 
\\

\cline{3-7}
 \multicolumn{1}{|l|}{} &
 &
 \multicolumn{1}{|l|}{Bandwagon} &
\multicolumn{1}{c|}{$0.06$} & 
\multicolumn{1}{c|}{$0.10$} &
\multicolumn{1}{c|}{$0.13$} & 
\multicolumn{1}{c|}{$0.14$}
\\

\hline
\multicolumn{1}{|l|}{\multirow{8}{*}{\em Yelp}} & 
\multicolumn{1}{l}{\multirow{4}{*}{NCF}} & 
% \multicolumn{1}{|l|}{{\sc Random}} &
% \multicolumn{1}{c|}{$8.32 (\pm 0.63)$} & 
% \multicolumn{1}{c|}{$5.00 (\pm 1.20)$} &
% \multicolumn{1}{c|}{$8.70 (\pm 0.47)$} & 
% \multicolumn{1}{c|}{$5.23 (\pm 0.85)$} &
% \multicolumn{1}{c|}{$9.10 (\pm 0.49)$} & 
% \multicolumn{1}{c|}{$5.00 (\pm 1.20)$}
% \\
% \cline{3-9}
% \multicolumn{1}{|l|}{} &
% &
\multicolumn{1}{|l|}{{DL-Attack}} & 
\multicolumn{1}{c|}{$\bf{0.27}$} & 
\multicolumn{1}{c|}{$0.30$} &
 \multicolumn{1}{c|}{$0.63$} & 
\multicolumn{1}{c|}{$0.73$} 
\\
\cline{3-7}
\multicolumn{1}{|l|}{} &
&
\multicolumn{1}{|l|}{{RAPU-R}} & 
\multicolumn{1}{c|}{$0.25$} &
\multicolumn{1}{c|}{$0.31$} &
\multicolumn{1}{c|}{$0.65$} & 
\multicolumn{1}{c|}{$0.74$} 
\\
\cline{3-7}
 \multicolumn{1}{|l|}{} &
 &
 \multicolumn{1}{|l|}{H-CARS} &
\multicolumn{1}{c|}{$0.26$} & 
\multicolumn{1}{c|}{$\bf{0.33}$} &
\multicolumn{1}{c|}{$\bf{0.66}$} & 
\multicolumn{1}{c|}{$\bf{0.76}$} 
\\
\cline{3-7}
 \multicolumn{1}{|l|}{} &
 &
 \multicolumn{1}{|l|}{Bandwagon} &
\multicolumn{1}{c|}{$0.05$} & 
\multicolumn{1}{c|}{$0.08$} &
\multicolumn{1}{c|}{$0.16$} & 
\multicolumn{1}{c|}{$0.21$}



\\
\cline{2-7}
\multicolumn{1}{|l|}{} & 
\multicolumn{1}{l}{\multirow{4}{*}{RCF}} & 
% \multicolumn{1}{|l|}{{\sc Random}} &
% \multicolumn{1}{c|}{${\bf5.81} (\pm 0.38)$} & \multicolumn{1}{c|}{${\bf4.59} (\pm 0.33)$} & 
% \multicolumn{1}{c|}{$7.52 (\pm 0.47)$} &
% \multicolumn{1}{c|}{$5.17 (\pm 1.09)$} &
% \multicolumn{1}{c|}{$8.19 (\pm 0.21)$} & 
% \multicolumn{1}{c|}{$8.20 (\pm 1.60)$} 
% \\
% \cline{3-9}
% \multicolumn{1}{|l|}{} &
% &
\multicolumn{1}{|l|}{{DL-Attack}} & 
 \multicolumn{1}{c|}{$\bf{0.24}$} &
\multicolumn{1}{c|}{$0.25$} &
 \multicolumn{1}{c|}{$0.56$} & 
\multicolumn{1}{c|}{$0.63$} 

\\
\cline{3-7}
\multicolumn{1}{|l|}{} &
&
\multicolumn{1}{|l|}{{RAPU-R}} & 
 \multicolumn{1}{c|}{$0.22$} & 
\multicolumn{1}{c|}{$0.24$} &
\multicolumn{1}{c|}{$0.59$} & 
\multicolumn{1}{c|}{$0.63$} 

\\
\cline{3-7}
 \multicolumn{1}{|l|}{} &
 &
 \multicolumn{1}{|l|}{H-CARS} &
\multicolumn{1}{c|}{$0.23$} & 
\multicolumn{1}{c|}{$\bf{0.26}$} &
\multicolumn{1}{c|}{$\bf{0.61}$} & 
\multicolumn{1}{c|}{$\bf{0.66}$} 
\\
\cline{3-7}
 \multicolumn{1}{|l|}{} &
 &
 \multicolumn{1}{|l|}{Bandwagon} &
\multicolumn{1}{c|}{$0.03$} & 
\multicolumn{1}{c|}{$0.04$} &
\multicolumn{1}{c|}{$0.12$} & 
\multicolumn{1}{c|}{$0.18$}
\\
\cline{2-7}
\hline
\end{tabular}
\quad
\begin{tabular}{lll|cccc|}
\cline{4-7}
& & & \multicolumn{4}{c|}{{\bf Percentage of Cotrolled Users}}
\\
\hline
 \multicolumn{1}{|l|}{\bf Dataset} & \multicolumn{1}{l}{\thead{Recommendation\\Model}} & \multicolumn{1}{|l|}{\thead{Attack\\Method}} & \multicolumn{1}{c|}{\thead{$0.5\%$}} & \multicolumn{1}{c|}{\thead{$1\%$}} & \multicolumn{1}{c|}{\thead{$3\%$}} & \multicolumn{1}{c|}{\thead{$5\%$}}
\\
\hline
\multicolumn{1}{|l|}{\multirow{8}{*}{\em MovieLens}} & 
\multicolumn{1}{l}{\multirow{4}{*}{NCF}} & 
% \multicolumn{1}{|l|}{{\sc Random}} &
% \multicolumn{1}{c|}{$8.32 (\pm 0.63)$} & 
% \multicolumn{1}{c|}{$5.00 (\pm 1.20)$} &
% \multicolumn{1}{c|}{$8.70 (\pm 0.47)$} & 
% \multicolumn{1}{c|}{$5.23 (\pm 0.85)$} &
% \multicolumn{1}{c|}{$9.10 (\pm 0.49)$} & 
% \multicolumn{1}{c|}{$5.00 (\pm 1.20)$}
% \\
% \cline{3-9}
% \multicolumn{1}{|l|}{} &
% &
\multicolumn{1}{|l|}{{DL-Attack}} & 
\multicolumn{1}{c|}{$0.12$} & 
\multicolumn{1}{c|}{$0.14$} &
 \multicolumn{1}{c|}{$0.21$} & 
\multicolumn{1}{c|}{$0.23$} 
\\
\cline{3-7}
\multicolumn{1}{|l|}{} &
&
\multicolumn{1}{|l|}{{RAPU-R}} & 
\multicolumn{1}{c|}{$0.10$} &
\multicolumn{1}{c|}{$0.14$} &
\multicolumn{1}{c|}{$0.23$} & 
\multicolumn{1}{c|}{$0.29$} 
\\
\cline{3-7}
 \multicolumn{1}{|l|}{} &
 &
 \multicolumn{1}{|l|}{H-CARS} &
\multicolumn{1}{c|}{$\bf{0.13}$} & 
\multicolumn{1}{c|}{$\bf{0.18}$} &
\multicolumn{1}{c|}{$\bf{0.29}$} & 
\multicolumn{1}{c|}{$\bf{0.35}$} 
\\
\cline{3-7}
 \multicolumn{1}{|l|}{} &
 &
 \multicolumn{1}{|l|}{Bandwagon} &
\multicolumn{1}{c|}{$0.02$} & 
\multicolumn{1}{c|}{$0.03$} &
\multicolumn{1}{c|}{$0.05$} & 
\multicolumn{1}{c|}{$0.10$}



\\
\cline{2-7}
\multicolumn{1}{|l|}{} & 
\multicolumn{1}{l}{\multirow{4}{*}{RCF}} & 
% \multicolumn{1}{|l|}{{\sc Random}} &
% \multicolumn{1}{c|}{${\bf5.81} (\pm 0.38)$} & \multicolumn{1}{c|}{${\bf4.59} (\pm 0.33)$} & 
% \multicolumn{1}{c|}{$7.52 (\pm 0.47)$} &
% \multicolumn{1}{c|}{$5.17 (\pm 1.09)$} &
% \multicolumn{1}{c|}{$8.19 (\pm 0.21)$} & 
% \multicolumn{1}{c|}{$8.20 (\pm 1.60)$} 
% \\
% \cline{3-9}
% \multicolumn{1}{|l|}{} &
% &
\multicolumn{1}{|l|}{{DL-Attack}} & 
 \multicolumn{1}{c|}{$\bf{0.06}$} &
\multicolumn{1}{c|}{$0.09$} &
 \multicolumn{1}{c|}{$0.17$} & 
\multicolumn{1}{c|}{$0.22$} 

\\
\cline{3-7}
\multicolumn{1}{|l|}{} &
&
\multicolumn{1}{|l|}{{RAPU-R}} & 
 \multicolumn{1}{c|}{$0.04$} & 
\multicolumn{1}{c|}{$0.08$} &
\multicolumn{1}{c|}{$0.17$} & 
\multicolumn{1}{c|}{$0.21$} 

\\
\cline{3-7}
\multicolumn{1}{|l|}{} &
&
\multicolumn{1}{|l|}{H-CARS} &
 \multicolumn{1}{c|}{$\bf{0.06}$} & 
\multicolumn{1}{c|}{$\bf{0.11}$} & 
\multicolumn{1}{c|}{$\bf{0.20}$} & 
\multicolumn{1}{c|}{$\bf{0.26}$} 
\\

\cline{3-7}
 \multicolumn{1}{|l|}{} &
 &
 \multicolumn{1}{|l|}{Bandwagon} &
\multicolumn{1}{c|}{$0.03$} & 
\multicolumn{1}{c|}{$0.03$} &
\multicolumn{1}{c|}{$0.05$} & 
\multicolumn{1}{c|}{$0.08$}
\\

\hline

\multicolumn{1}{|l|}{\multirow{8}{*}{\em Yelp}} & 
\multicolumn{1}{l}{\multirow{4}{*}{NCF}} & 
% \multicolumn{1}{|l|}{{\sc Random}} &
% \multicolumn{1}{c|}{$8.32 (\pm 0.63)$} & 
% \multicolumn{1}{c|}{$5.00 (\pm 1.20)$} &
% \multicolumn{1}{c|}{$8.70 (\pm 0.47)$} & 
% \multicolumn{1}{c|}{$5.23 (\pm 0.85)$} &
% \multicolumn{1}{c|}{$9.10 (\pm 0.49)$} & 
% \multicolumn{1}{c|}{$5.00 (\pm 1.20)$}
% \\
% \cline{3-9}
% \multicolumn{1}{|l|}{} &
% &
\multicolumn{1}{|l|}{{DL-Attack}} & 
 \multicolumn{1}{c|}{$0.05$} &
\multicolumn{1}{c|}{$0.06$} &
 \multicolumn{1}{c|}{$0.09$} & 
\multicolumn{1}{c|}{$0.11$} 

\\
\cline{3-7}
\multicolumn{1}{|l|}{} &
&
\multicolumn{1}{|l|}{{RAPU-R}} & 
 \multicolumn{1}{c|}{$0.05$} & 
\multicolumn{1}{c|}{$0.05$} &
\multicolumn{1}{c|}{$0.09$} & 
\multicolumn{1}{c|}{$0.12$} 

\\
\cline{3-7}
\multicolumn{1}{|l|}{} &
&
\multicolumn{1}{|l|}{H-CARS} &
 \multicolumn{1}{c|}{$\bf{0.06}$} & 
\multicolumn{1}{c|}{$\bf{0.08}$} & 
\multicolumn{1}{c|}{$\bf{0.12}$} & 
\multicolumn{1}{c|}{$\bf{0.16}$} 
\\

\cline{3-7}
 \multicolumn{1}{|l|}{} &
 &
 \multicolumn{1}{|l|}{Bandwagon} &
\multicolumn{1}{c|}{$0.01$} & 
\multicolumn{1}{c|}{$0.02$} &
\multicolumn{1}{c|}{$0.06$} & 
\multicolumn{1}{c|}{$0.08$}
\\
\cline{2-7}

\multicolumn{1}{|l|}{} & 
\multicolumn{1}{l}{\multirow{4}{*}{RCF}} & 
% \multicolumn{1}{|l|}{{\sc Random}} &
% \multicolumn{1}{c|}{${\bf5.81} (\pm 0.38)$} & \multicolumn{1}{c|}{${\bf4.59} (\pm 0.33)$} & 
% \multicolumn{1}{c|}{$7.52 (\pm 0.47)$} &
% \multicolumn{1}{c|}{$5.17 (\pm 1.09)$} &
% \multicolumn{1}{c|}{$8.19 (\pm 0.21)$} & 
% \multicolumn{1}{c|}{$8.20 (\pm 1.60)$} 
% \\
% \cline{3-9}
% \multicolumn{1}{|l|}{} &
% &
\multicolumn{1}{|l|}{{DL-Attack}} & 
 \multicolumn{1}{c|}{$0.06$} &
\multicolumn{1}{c|}{$0.08$} &
 \multicolumn{1}{c|}{$0.13$} & 
\multicolumn{1}{c|}{$0.15$} 

\\
\cline{3-7}
\multicolumn{1}{|l|}{} &
&
\multicolumn{1}{|l|}{{RAPU-R}} & 
 \multicolumn{1}{c|}{$0.06$} & 
\multicolumn{1}{c|}{$0.09$} &
\multicolumn{1}{c|}{$0.13$} & 
\multicolumn{1}{c|}{$0.16$} 

\\
\cline{3-7}
\multicolumn{1}{|l|}{} &
&
\multicolumn{1}{|l|}{H-CARS} &
 \multicolumn{1}{c|}{$\bf{0.07}$} & 
\multicolumn{1}{c|}{$\bf{0.10}$} & 
\multicolumn{1}{c|}{$\bf{0.15}$} & 
\multicolumn{1}{c|}{$\bf{0.20}$} 
\\

\cline{3-7}
 \multicolumn{1}{|l|}{} &
 &
 \multicolumn{1}{|l|}{Bandwagon} &
\multicolumn{1}{c|}{$0.02$} & 
\multicolumn{1}{c|}{$0.03$} &
\multicolumn{1}{c|}{$0.05$} & 
\multicolumn{1}{c|}{$0.10$}
\\
\cline{2-7}

\hline


\end{tabular}
}
\end{table*}

==> Attack_result30.tex <==
\begin{table*}[ht!]
\caption{\label{tab:Result30}
HR@10$\times$100 for different attacks with $30\%$ training data on two datasets (best performance in bold).
}
\vspace{-2mm}
\scalebox{0.75}{
\centering
\begin{tabular}{lll|cccc|}
\cline{4-7}
& & & \multicolumn{4}{c|}{{\bf Percentage of Cotrolled Users}}
\\
\hline
 \multicolumn{1}{|l|}{\bf Dataset} & \multicolumn{1}{l}{\thead{Recommendation\\Model}} & \multicolumn{1}{|l|}{\thead{Attack\\Method}} & \multicolumn{1}{c|}{\thead{$0.5\%$}} & \multicolumn{1}{c|}{\thead{$1\%$}} & \multicolumn{1}{c|}{\thead{$3\%$}} & \multicolumn{1}{c|}{\thead{$5\%$}}
\\
\hline
\multicolumn{1}{|l|}{\multirow{9}{*}{\em MovieLens}} & 
\multicolumn{1}{l}{\multirow{4}{*}{NCF}} & 
% \multicolumn{1}{|l|}{{\sc Random}} &
% \multicolumn{1}{c|}{$8.32 (\pm 0.63)$} & 
% \multicolumn{1}{c|}{$5.00 (\pm 1.20)$} &
% \multicolumn{1}{c|}{$8.70 (\pm 0.47)$} & 
% \multicolumn{1}{c|}{$5.23 (\pm 0.85)$} &
% \multicolumn{1}{c|}{$9.10 (\pm 0.49)$} & 
% \multicolumn{1}{c|}{$5.00 (\pm 1.20)$}
% \\
% \cline{3-9}
% \multicolumn{1}{|l|}{} &
% &
\multicolumn{1}{|l|}{{\sc DL-Attack}} & 
\multicolumn{1}{c|}{$0.0012$} & 
\multicolumn{1}{c|}{$0.0014$} &
 \multicolumn{1}{c|}{$0.0021$} & 
\multicolumn{1}{c|}{$0.0023$} 
\\
\cline{3-7}
\multicolumn{1}{|l|}{} &
&
\multicolumn{1}{|l|}{{\sc RAPU-R}} & 
\multicolumn{1}{c|}{$0.0010$} &
\multicolumn{1}{c|}{$0.0014$} &
\multicolumn{1}{c|}{$0.0023$} & 
\multicolumn{1}{c|}{$0.0029$} 
\\
\cline{3-7}
 \multicolumn{1}{|l|}{} &
 &
 \multicolumn{1}{|l|}{\sc H-CARS} &
\multicolumn{1}{c|}{$0.0013$} & 
\multicolumn{1}{c|}{$0.0018$} &
\multicolumn{1}{c|}{$0.0029$} & 
\multicolumn{1}{c|}{$0.0035$} 
\\
\cline{3-7}
 \multicolumn{1}{|l|}{} &
 &
 \multicolumn{1}{|l|}{\sc Bandwagon} &
\multicolumn{1}{c|}{$0.0002$} & 
\multicolumn{1}{c|}{$0.0003$} &
\multicolumn{1}{c|}{$0.0005$} & 
\multicolumn{1}{c|}{$0.0010$}



\\
\cline{2-7}
\multicolumn{1}{|l|}{} & 
\multicolumn{1}{l}{\multirow{4}{*}{RCF}} & 
% \multicolumn{1}{|l|}{{\sc Random}} &
% \multicolumn{1}{c|}{${\bf5.81} (\pm 0.38)$} & \multicolumn{1}{c|}{${\bf4.59} (\pm 0.33)$} & 
% \multicolumn{1}{c|}{$7.52 (\pm 0.47)$} &
% \multicolumn{1}{c|}{$5.17 (\pm 1.09)$} &
% \multicolumn{1}{c|}{$8.19 (\pm 0.21)$} & 
% \multicolumn{1}{c|}{$8.20 (\pm 1.60)$} 
% \\
% \cline{3-9}
% \multicolumn{1}{|l|}{} &
% &
\multicolumn{1}{|l|}{{\sc DL-Attack}} & 
 \multicolumn{1}{c|}{$0.0006$} &
\multicolumn{1}{c|}{$0.0009$} &
 \multicolumn{1}{c|}{$0.0017$} & 
\multicolumn{1}{c|}{$0.0022$} 

\\
\cline{3-7}
\multicolumn{1}{|l|}{} &
&
\multicolumn{1}{|l|}{{\sc RAPU-R}} & 
 \multicolumn{1}{c|}{$0.0004$} & 
\multicolumn{1}{c|}{$0.0008$} &
\multicolumn{1}{c|}{$0.0017$} & 
\multicolumn{1}{c|}{$0.0021$} 

\\
\cline{3-7}
\multicolumn{1}{|l|}{} &
&
\multicolumn{1}{|l|}{\sc H-CARS} &
 \multicolumn{1}{c|}{$0.0006$} & 
\multicolumn{1}{c|}{$0.0011$} & 
\multicolumn{1}{c|}{$0.0020$} & 
\multicolumn{1}{c|}{$0.0026$} 
\\

\cline{3-7}
 \multicolumn{1}{|l|}{} &
 &
 \multicolumn{1}{|l|}{\sc Bandwagon} &
\multicolumn{1}{c|}{$0.0003$} & 
\multicolumn{1}{c|}{$0.0003$} &
\multicolumn{1}{c|}{$0.0005$} & 
\multicolumn{1}{c|}{$0.0008$}
\\
\cline{2-7}

\hline

\multicolumn{1}{|l|}{\multirow{9}{*}{\em Yelp}} & 
\multicolumn{1}{l}{\multirow{4}{*}{NCF}} & 
% \multicolumn{1}{|l|}{{\sc Random}} &
% \multicolumn{1}{c|}{$8.32 (\pm 0.63)$} & 
% \multicolumn{1}{c|}{$5.00 (\pm 1.20)$} &
% \multicolumn{1}{c|}{$8.70 (\pm 0.47)$} & 
% \multicolumn{1}{c|}{$5.23 (\pm 0.85)$} &
% \multicolumn{1}{c|}{$9.10 (\pm 0.49)$} & 
% \multicolumn{1}{c|}{$5.00 (\pm 1.20)$}
% \\
% \cline{3-9}
% \multicolumn{1}{|l|}{} &
% &
\multicolumn{1}{|l|}{{\sc DL-Attack}} & 
 \multicolumn{1}{c|}{$0.0005$} &
\multicolumn{1}{c|}{$0.0006$} &
 \multicolumn{1}{c|}{$0.009$} & 
\multicolumn{1}{c|}{$0.0011$} 

\\
\cline{3-7}
\multicolumn{1}{|l|}{} &
&
\multicolumn{1}{|l|}{{\sc RAPU-R}} & 
 \multicolumn{1}{c|}{$0.0005$} & 
\multicolumn{1}{c|}{$0.0005$} &
\multicolumn{1}{c|}{$0.009$} & 
\multicolumn{1}{c|}{$0.0012$} 

\\
\cline{3-7}
\multicolumn{1}{|l|}{} &
&
\multicolumn{1}{|l|}{\sc H-CARS} &
 \multicolumn{1}{c|}{$0.0006$} & 
\multicolumn{1}{c|}{$0.0008$} & 
\multicolumn{1}{c|}{$0.0012$} & 
\multicolumn{1}{c|}{$0.0016$} 
\\

\cline{3-7}
 \multicolumn{1}{|l|}{} &
 &
 \multicolumn{1}{|l|}{\sc Bandwagon} &
\multicolumn{1}{c|}{$0.0001$} & 
\multicolumn{1}{c|}{$0.0002$} &
\multicolumn{1}{c|}{$0.0006$} & 
\multicolumn{1}{c|}{$0.0008$}
\\
\cline{2-7}

\multicolumn{1}{|l|}{} & 
\multicolumn{1}{l}{\multirow{4}{*}{RCF}} & 
% \multicolumn{1}{|l|}{{\sc Random}} &
% \multicolumn{1}{c|}{${\bf5.81} (\pm 0.38)$} & \multicolumn{1}{c|}{${\bf4.59} (\pm 0.33)$} & 
% \multicolumn{1}{c|}{$7.52 (\pm 0.47)$} &
% \multicolumn{1}{c|}{$5.17 (\pm 1.09)$} &
% \multicolumn{1}{c|}{$8.19 (\pm 0.21)$} & 
% \multicolumn{1}{c|}{$8.20 (\pm 1.60)$} 
% \\
% \cline{3-9}
% \multicolumn{1}{|l|}{} &
% &
\multicolumn{1}{|l|}{{\sc DL-Attack}} & 
 \multicolumn{1}{c|}{$0.0006$} &
\multicolumn{1}{c|}{$0.0008$} &
 \multicolumn{1}{c|}{$0.0013$} & 
\multicolumn{1}{c|}{$0.0015$} 

\\
\cline{3-7}
\multicolumn{1}{|l|}{} &
&
\multicolumn{1}{|l|}{{\sc RAPU-R}} & 
 \multicolumn{1}{c|}{$0.0006$} & 
\multicolumn{1}{c|}{$0.0009$} &
\multicolumn{1}{c|}{$0.0013$} & 
\multicolumn{1}{c|}{$0.0016$} 

\\
\cline{3-7}
\multicolumn{1}{|l|}{} &
&
\multicolumn{1}{|l|}{\sc H-CARS} &
 \multicolumn{1}{c|}{$0.0007$} & 
\multicolumn{1}{c|}{$0.0010$} & 
\multicolumn{1}{c|}{$0.0015$} & 
\multicolumn{1}{c|}{$0.0020$} 
\\

\cline{3-7}
 \multicolumn{1}{|l|}{} &
 &
 \multicolumn{1}{|l|}{\sc Bandwagon} &
\multicolumn{1}{c|}{$0.0002$} & 
\multicolumn{1}{c|}{$0.0003$} &
\multicolumn{1}{c|}{$0.0005$} & 
\multicolumn{1}{c|}{$0.0010$}
\\
\cline{2-7}

\hline


\end{tabular}
}
\end{table*}

==> Related.tex <==
\section{Related Work}
\label{sec:Relate}


\subsection{Unlearning for LLM-based Recommendation.} 
Traditional recommendation unlearning methods, such as RecEraser \cite{chen2022recommendation} and AltEraser \cite{liu2022forgetting}, focus on partitioning collaborative data to safeguard privacy but are ill-suited for the massive parameter space of Large Language Models (LLMs). Conversely, general LLM unlearning often relies on approximate methods like gradient ascent \cite{yao2024large} or in-context label flipping, which frequently trigger catastrophic forgetting and degrade recommendation utility. To mitigate these issues, recent LLMRec-specific frameworks have adopted parameter-efficient fine-tuning (PEFT) \cite{zhang2025parameter}. E2URec\cite{wang2025towards} introduces a teacher-student architecture to guide the unlearning process via minimal LoRA updates, while the Adapter Partition and Aggregation (APA) framework employs data sharding and adapter retraining to achieve exact unlearning. However, these methods typically treat the model as a black box and apply uniform updates, leading to gradient conflicts between forgetting and retaining objectives. Our framework, \textsf{CURE}, addresses this by moving beyond uniform updates to a more granular, component-specific optimization strategy.

\subsection{Circuit Discovery}
Circuit discovery is the task of identifying sparse, functional subgraphs within a neural network that are causally responsible for implementing specific capabilities or behaviors \cite{conmy2023towards}. This paradigm shifts the focus from global parameter analysis to localizing the "essential computation" for a particular task. Early manual investigations, such as those by \cite{wang2022interpretability} and \cite{hanna2023does}, utilized causal mediation analysis and activation patching to uncover circuits for indirect object identification and mathematical reasoning in small-scale models. However, the manual search space grows exponentially with model depth, leading to the development of automated frameworks. ACDC \cite{conmy2023towards} automates circuit identification by recursively pruning edges based on their contribution to model faithfulness. While effective, its reliance on iterative testing renders it too computationally expensive for the scale of modern LLMs. To overcome this, Subnetwork Probing \cite{cao2021low} treats circuit identification as a mask-learning problem, optimizing for both fidelity and sparsity. More recently, \textbf{Edge Attribution Patching (EAP)} \cite{syed2024attribution} has emerged as a high-efficiency alternative, leveraging gradient-based importance scores to approximate the effect of interventions with minimal forward and backward passes. While these techniques have primarily been applied to linguistic benchmarks, we leverage circuit discovery techniques to extract the core circuits underlying item recommendation in LLM based recommendation. This structural decomposition provides the necessary transparency to disentangle the model into \textit{forget-specific} and \textit{retain-specific} modules, bridging the gap between mechanistic interpretability and trustworthy unlearning in recommender systems.

\subsection{Gradient Conflicts in Unlearning}
The optimization of unlearning objectives often mirrors the challenges of multi-task learning, where a model must simultaneously satisfy competing goals. In the context of unlearning, a fundamental tension exists between the \textit{forgetting} objective (erasing specific data) and the \textit{retaining} objective (maintaining model utility) \cite{patel2025learning}. Previous studies have identified that these dual goals frequently lead to detrimental gradient interference, where the update direction for one task adversely impacts the other \cite{yu2020gradient}. 
While PCGrad \cite{yu2020gradient} introduced a model-agnostic ``gradient surgery'' approach—projecting conflicting gradients onto their respective normal planes—this method does not account for the unique functional structure of LLMs. Recent analysis in BLUR \cite{reisizadeh2025blur} shows that these gradient conflicts are even more severe in Large Language Models (LLMs). This complexity requires specialized optimization strategies to ensure that forgetting specific data does not accidentally damage the model's performance on remaining tasks. Our work, \textsf{CURE}, builds on these insights by using circuit discovery to physically isolate the parameters where these conflicts occur, allowing for a more targeted resolution than previous gradient-projection methods.


\section{Conclusion}
In this paper, we propose CURE, a circuit-aware unlearning framework that addresses the challenges of gradient conflicts in LLMRec unlearning. By leveraging mechanistic interpretability to disentangle computational circuits into functionally distinct modules, CURE enables precise, task-specific parameter updates that effectively remove sensitive information while preserving model utility. Our evaluation demonstrates that CURE outperforms state-of-the-art baselines with an $18\%$ improvement in unlearning efficiency and a $6\%$ gain in utility, while achieving a $3.5\times$ speedup. By shifting from black-box updates to transparent, circuit-level interventions, CURE provides a robust and efficient solution for privacy-preserving recommendation.


==> ablation.tex <==
\section{Ablation Study}
\label{sec:ablation}



==> abstract.tex <==
\begin{abstract}
Recent advances in large language model(LLMs) offer new opportunities for recommender systems by capturing user interest and item characteristics through rich semantic understanding and reasoning. With growing emphasis on privacy regulations, the inclusion of user data in LLMs-based Recommendation(LLM-Rec) raises privacy concerns, and unlearning algorithms thereby become critical in real-world application. 



\\
In this work, we 
\end{abstract}

==> conclusion.tex <==
\section{Conclusion and Future Work}
\label{sec:conclusion}
%In this work, we presented H-CARS, the first poisoning attack to recommender systems that exploits vulnerabilities induced by counterfactual explanations. 


We presented a novel approach, H-CARS, that exploits the vulnerabilities induced by counterfactual explanations to launch a poisoning attack on recommender systems. To the best of our knowledge, this is the first such attack proposed in the literature. Our experiments demonstrate that H-CARS is effective, highlighting the importance of considering the security implications of using explainability methods in recommender systems. Future research should explore the potential impact of such attacks on the integrity of the recommender system, as well as develop stronger defenses to mitigate risks in explainable recommender systems.

==> evaluation.tex <==
\section{Worst-Case Evaluation}
\label{sec:Preliminary}

==> intro_xiangguo_FIY.tex <==

% \xg{Here are some suggestions when I read the original introduction: 

% A. Shift from “related-work-first” to “problem-first”. The current draft starts by classifying existing methods (approx vs exact). That reads like a survey and discourage us conitnuing reading.

% B. Make the challenge statements concrete and highlith them.

% C. Make circuit-aware motivation explicit and central. Right now circuits appear suddenly. Add a bridge sentence before introducing CURE, like: “This motivates a fine-grained, circuit-aware unlearning strategy: identify the computation pathways encoding target information, then update only those responsible components.” That makes the “why circuits” feel inevitable.

% D. Contribution bullets must match what was introduced earlier. Yang’s comment is correct: contribution 1 and 3 weren’t prepared well. Fix it by either: In intro body, explicitly preview counterfactual prompts + worst-case protocol, then contributions list. or Remove contribution 3 from the main contribution list and mention it as “evaluation protocol” later.

% E. Replace abstract “approximate vs exact” with one sentence only. You can keep the classification, but compress to a single sentence: “Existing approaches either retrain affected shards (often infeasible for deployed LLMRec) or perform approximate unlearning via loss re-weighting/distillation.” Then immediately pivot to the actual challenge: conflict + opacity.

% }




% \section{FYI: Introduction (from Xiangguo)}
% % Large Language Models (LLMs) are increasingly adopted as recommender systems (LLMRec), where recommendation is formulated as instruction-following: given a user’s historical interactions and a candidate item, the model reasons about preference and generates a decision (e.g., “Yes/No”) with supporting semantics. 

% Compared to conventional recommenders, LLMRec offers two attractive advantages: it can exploit rich open-world knowledge to better interpret item descriptions and user intent, and it can perform multi-step reasoning to model complex preference patterns. 

% These strengths, however, also expose a new risk surface: LLMRec is fine-tuned on user behavior logs that may contain sensitive information (e.g., purchase records, browsing traces), and the resulting model may inadvertently memorize or be manipulated by maliciously injected data. As LLMRec becomes deployed in real systems, the ability to reliably remove the influence of specified user data from a trained model—i.e., recommendation unlearning—becomes a practical requirement for privacy compliance and trustworthy deployment.


% The central goal of unlearning is conceptually simple: after receiving a deletion request, the updated model should behave as if the sensitive data had never been used for training, while maintaining recommendation quality on the remaining data. Achieving this goal in LLMRec is challenging for three reasons:
% \begin{itemize}
%     \item \textbf{First, retraining from scratch on the remaining data is often infeasible.} LLMRec typically relies on costly instruction tuning over long prompts and large models; deletion requests may arrive continuously and require fast model updates, making repeated retraining prohibitively expensive. In addition, a deployed system may not preserve full training pipelines or complete retention data, further limiting the feasibility of “exact” retraining-based solutions. 
%    \item \textbf{Second, existing approximate unlearning methods face a fundamental optimization dilemma.} Most approaches formulate unlearning as minimizing a weighted combination of a forgetting objective (to suppress the influence of the forget set) and a retention objective (to preserve utility on the retain set). Yet, in LLMRec this coupling is particularly fragile: forgetting and retention frequently induce opposing gradient directions at fine granularity, so updates that improve forgetting can immediately degrade utility, while utility-preserving updates can protect exactly what should be forgotten. This gradient conflict often forces practitioners into unstable hyperparameter tuning and results in either insufficient forgetting or noticeable utility loss.
%    \item \textbf{Third, current unlearning procedures remain largely black-box.} They update model parameters globally without explicit understanding of which internal computations encode the targeted information. As a result, unlearning becomes difficult to interpret, difficult to control, and difficult to trust—especially in sensitive scenarios where we need to verify what was removed and what was preserved.
% \end{itemize}

% This paper argues that the above challenges stem from a common root cause: knowledge in LLMRec is not uniformly distributed across parameters; it is activated through sparse computational pathways (``circuits'') conditioned on the prompt. Different subsets of the model contribute to the final recommendation decision depending on the user’s history, candidate item, and prompt structure. Crucially, gradient conflicts arise when the circuits responsible for forgetting and those needed for retention are entangled, i.e., they share internal components that are simultaneously pushed in opposite directions. This observation suggests that a model-wide, semantically agnostic update is inherently misaligned with the unlearning objective. Instead, effective and trustworthy unlearning should be circuit-aware: identify which circuits are responsible for forget/retain behaviors, then update only the components that truly require modification while protecting utility-critical pathways.

% Motivated by this insight, we propose CURE, a circuit-aware unlearning framework tailored for LLMRec. CURE decomposes unlearning into two stages. \textbf{First}, it performs circuit extraction to localize the internal computation pathways most responsible for the forget and retain sets. To improve localization under long prompts—a common setting in LLMRec—we introduce a graph-aware counterfactual prompt construction strategy based on the user–item interaction graph, which enables more precise activation patching and circuit identification. \textbf{Second}, CURE conducts selective updating guided by extracted circuits: model components are categorized as forget-specific, retain-specific, or shared, and are updated with distinct policies that explicitly mitigate gradient conflicts. This results in targeted, semantically grounded parameter changes that enhance forgetting effectiveness while preserving recommendation utility and improving the interpretability of the unlearning process.


% Our contributions are threefold:
% \begin{itemize}
%     \item We introduce a circuit-based perspective for understanding and addressing gradient conflicts in LLMRec unlearning, connecting unlearning failures to circuit entanglement.
%     \item We propose CURE, a two-stage circuit-aware unlearning framework with graph-aware counterfactual activation patching and component-level selective updating to reduce gradient conflicts and improve trustworthiness.
%     \item We design a worst-case forgetting evaluation protocol for LLMRec, aiming to stress-test unlearning robustness beyond average-case metrics, and empirically demonstrate the effectiveness of CURE on real-world datasets.
% \end{itemize}


==> related.tex <==
\section{Related Work}
\label{sec:related}


==> table.tex <==
\begin{table*}[ht]
\scalebox{0.6}{
\centering
%\begin{tabular}{lll|cc|cc|cc|}
\begin{tabular}{lll|cc|cc|cc|cc|cc|cc|}
%\cline{4-9}
\cline{4-15}
% & & & \multicolumn{2}{c|}{{\bf Top-$10$}} & \multicolumn{2}{c|}{{\bf Top-$15$}} & \multicolumn{2}{c|}{{\bf Top-$20$}}
& & & \multicolumn{4}{c|}{{\bf Top-$10$}} & \multicolumn{4}{c|}{{\bf Top-$15$}} & \multicolumn{4}{c|}{{\bf Top-$20$}}
\\
%\cline{4-9}
\cline{4-15}
% & & & \multicolumn{1}{c|}{{\bf factual}} & \multicolumn{1}{c|}{{\bf counterfactual}} & \multicolumn{1}{c|}{{\bf factual}} & \multicolumn{1}{c|}{{\bf counterfactual}} & \multicolumn{1}{c|}{{\bf factual}} & \multicolumn{1}{c|}{{\bf counterfactual}}
& & & \multicolumn{2}{c|}{{\bf factual}} & \multicolumn{2}{c|}{{\bf counterfactual}} & \multicolumn{2}{c|}{{\bf factual}} & \multicolumn{2}{c|}{{\bf counterfactual}} & \multicolumn{2}{c|}{{\bf factual}} & \multicolumn{2}{c|}{{\bf counterfactual}}
\\
\hline
% \multicolumn{1}{|l|}{\bf Dataset} & \multicolumn{1}{l|}{\thead{Recommendation\\Model}} & \multicolumn{1}{l|}{\thead{Explanation\\Method}} & \multicolumn{1}{c|}{\thead{\bf PS$\uparrow$ / EC$\downarrow$}} & \multicolumn{1}{c|}{\thead{\bf PN$\uparrow$ / EC$\downarrow$}} & \multicolumn{1}{c|}{\thead{\bf PS$\uparrow$ / EC$\downarrow$}} & \multicolumn{1}{c|}{\thead{\bf PN$\uparrow$ / EC$\downarrow$}} & \multicolumn{1}{c|}{\thead{\bf PS$\uparrow$ / EC$\downarrow$}} & \multicolumn{1}{c|}{\thead{\bf PN$\uparrow$ / EC$\downarrow$}}
\multicolumn{1}{|l|}{\bf Dataset} & \multicolumn{1}{l}{\thead{Recommendation\\Model}} & \multicolumn{1}{|l|}{\thead{Explanation\\Method}} & \multicolumn{1}{c|}{\bf PS} & \multicolumn{1}{c|}{\bf EC} & \multicolumn{1}{c|}{\bf PN} & \multicolumn{1}{c|}{\bf EC} &
\multicolumn{1}{c|}{\bf PS} & \multicolumn{1}{c|}{\bf EC} & \multicolumn{1}{c|}{\bf PN} & \multicolumn{1}{c|}{\bf EC} &
\multicolumn{1}{c|}{\bf PS} & \multicolumn{1}{c|}{\bf EC} & \multicolumn{1}{c|}{\bf PN} & \multicolumn{1}{c|}{\bf EC}
\\
\hline
% LastFM
\multicolumn{1}{|l|}{\multirow{12}{*}{\em LastFM}} & 
\multicolumn{1}{l}{\multirow{4}{*}{LightGCN}} & 
\multicolumn{1}{|l|}{GREASE} &
\multicolumn{1}{l|}{${\bf0.62} (\pm 0.05)$} & \multicolumn{1}{c|}{${\bf5.91} (\pm 0.70)$} & \multicolumn{1}{c|}{${\bf0.87} (\pm 0.02)$} &
\multicolumn{1}{c|}{${\bf3.98} (\pm 0.26)$} &
\multicolumn{1}{l|}{${\bf0.56} (\pm 0.05)$} & \multicolumn{1}{c|}{${\bf5.31} (\pm 0.58)$} & \multicolumn{1}{c|}{${\bf0.85} (\pm 0.07)$} &
\multicolumn{1}{c|}{${\bf4.17} (\pm 0.38)$} &
\multicolumn{1}{c|}{${\bf0.55} (\pm 0.08)$} & \multicolumn{1}{c|}{${\bf5.67} (\pm 0.75)$} & \multicolumn{1}{c|}{$\mathbf{0.82} (\pm 0.08)$} &
\multicolumn{1}{c|}{$\mathbf{4.58} (\pm 0.45)$}
\\
\cline{3-15}
\multicolumn{1}{|l|}{} &
% \multicolumn{1}{l|}{LightGCN} &
&
\multicolumn{1}{|l|}{{\sc PGExplainer}} & 
\multicolumn{1}{l|}{$0.57 (\pm 0.03)$} & \multicolumn{1}{c|}{$6.30 (\pm 0.40)$} & \multicolumn{1}{c|}{$0.85 (\pm 0.04)$} &
\multicolumn{1}{c|}{$4.37 (\pm 0.32)$} &
\multicolumn{1}{l|}{$0.54 (\pm 0.03)$} & \multicolumn{1}{c|}{$6.35 (\pm 0.43)$} & \multicolumn{1}{c|}{$0.82 (\pm 0.05)$} &
\multicolumn{1}{c|}{$5.39 (\pm 0.35)$} &
\multicolumn{1}{c|}{$0.49 (\pm 0.06)$} & \multicolumn{1}{c|}{$6.11 (\pm 0.70)$} & \multicolumn{1}{c|}{$\mathbf{0.82} (\pm 0.07)$} &
\multicolumn{1}{c|}{$4.66 (\pm 0.45)$}
\\
\cline{3-15}
\multicolumn{1}{|l|}{} &
% \multicolumn{1}{l|}{LightGCN} &
&
\multicolumn{1}{|l|}{{\sc PersonalRank}} & 
\multicolumn{1}{l|}{$0.58 (\pm 0.03)$} & \multicolumn{1}{c|}{$6.68 (\pm 0.36)$} & \multicolumn{1}{c|}{$0.85 (\pm 0.06)$} &
\multicolumn{1}{c|}{$4.73 (\pm 0.53)$} &
\multicolumn{1}{l|}{$0.55 (\pm 0.03)$} & \multicolumn{1}{c|}{$6.87 (\pm 0.41)$} & \multicolumn{1}{c|}{$0.77 (\pm 0.05)$} &
\multicolumn{1}{c|}{$5.23 (\pm 0.29)$} &
\multicolumn{1}{c|}{$0.53 (\pm 0.05)$} &
\multicolumn{1}{c|}{$7.31 (\pm 0.52)$} & \multicolumn{1}{c|}{$0.76 (\pm 0.07)$} &
\multicolumn{1}{c|}{$5.79 (\pm 0.32)$}
\\
\cline{3-15}
 \multicolumn{1}{|l|}{} &
% \multicolumn{1}{l|}{} & 
&
\multicolumn{1}{|l|}{{\sc Random}} &
\multicolumn{1}{l|}{$0.07 (\pm 0.02)$} & \multicolumn{1}{c|}{$8.32 (\pm 0.63)$} & \multicolumn{1}{c|}{$0.19 (\pm 0.03)$} &
\multicolumn{1}{c|}{$5.00 (\pm 1.20)$} &
\multicolumn{1}{l|}{$0.09 (\pm 0.04)$} & \multicolumn{1}{c|}{$8.70 (\pm 0.47)$} & \multicolumn{1}{c|}{$0.13 (\pm 0.03)$} &
\multicolumn{1}{c|}{$5.23 (\pm 0.85)$} &
\multicolumn{1}{c|}{$0.06 (\pm 0.02)$} &
\multicolumn{1}{c|}{$9.10 (\pm 0.49)$} & \multicolumn{1}{c|}{$0.19 (\pm 0.03)$} & \multicolumn{1}{c|}{$5.00 (\pm 1.20)$}
\\
\cline{2-15}
\multicolumn{1}{|l|}{} & 
\multicolumn{1}{l}{\multirow{4}{*}{NGCF}} & 
\multicolumn{1}{|l|}{GREASE} &
\multicolumn{1}{l|}{$0.63 (\pm 0.05)$} & \multicolumn{1}{c|}{$6.50 (\pm 0.83)$} & \multicolumn{1}{c|}{$0.92 (\pm 0.06)$} &
\multicolumn{1}{c|}{$4.90 (\pm 0.35    )$} &
\multicolumn{1}{l|}{$0.55 (\pm 0.05)$} & \multicolumn{1}{c|}{$6.35 (\pm 0.83)$} & \multicolumn{1}{c|}{$0.88 (\pm 0.07)$} &
\multicolumn{1}{c|}{$4.26 (\pm 0.34)$} &
\multicolumn{1}{c|}{$\mathbf{0.70} (\pm 0.06)$} & \multicolumn{1}{c|}{$\mathbf{6.30} (\pm 0.82)$} & \multicolumn{1}{c|}{$\mathbf{0.86} (\pm 0.09)$} & \multicolumn{1}{c|}{$\mathbf{5.01} (\pm 0.46)$}
\\
\cline{3-15}
\multicolumn{1}{|l|}{} &
% \multicolumn{1}{l|}{LightGCN} &
&
\multicolumn{1}{|l|}{{\sc PGExplainer}} & 
\multicolumn{1}{l|}{$0.61 (\pm 0.04)$} & \multicolumn{1}{c|}{$6.70 (\pm 0.82)$} & \multicolumn{1}{c|}{$0.90 (\pm 0.05)$} &
\multicolumn{1}{c|}{$5.39 (\pm 0.43)$} &
\multicolumn{1}{l|}{$0.52 (\pm 0.06)$} & \multicolumn{1}{c|}{$6.66 (\pm 0.78)$} & \multicolumn{1}{c|}{$0.86 (\pm 0.05)$} &
\multicolumn{1}{c|}{$4.68 (\pm 0.35)$} &
\multicolumn{1}{c|}{$0.68 (\pm 0.07)$} &
\multicolumn{1}{c|}{$6.42 (\pm 0.79)$} & \multicolumn{1}{c|}{$0.85 (\pm 0.05)$} &
\multicolumn{1}{c|}{$5.32 (\pm 0.43)$}
\\
\cline{3-15}
%\multicolumn{1}{|l|}{\textit{LastFM}} &
\multicolumn{1}{|l|}{} &
%\multicolumn{1}{l|}{NGCF} & 
&
\multicolumn{1}{|l|}{{\sc PersonalRank}} & 
\multicolumn{1}{l|}{$0.59 (\pm 0.05)$} & \multicolumn{1}{c|}{$6.68 (\pm 0.36)$} & \multicolumn{1}{c|}{$0.88 (\pm 0.03)$} &
\multicolumn{1}{c|}{$5.37 (\pm 0.42)$} &
\multicolumn{1}{l|}{$0.50 (\pm 0.04)$} & \multicolumn{1}{c|}{$6.68 (\pm 0.79)$} & \multicolumn{1}{c|}{$0.85 (\pm 0.05)$} &
\multicolumn{1}{c|}{$4.63 (\pm 0.39)$} &
\multicolumn{1}{c|}{$0.58 (\pm 0.02)$} & \multicolumn{1}{c|}{$6.68 (\pm 0.36)$} & \multicolumn{1}{c|}{$0.83 (\pm 0.03)$} & \multicolumn{1}{c|}{$7.21 (\pm 0.51)$}
\\
\cline{3-15}
\multicolumn{1}{|l|}{} &
% \multicolumn{1}{l|}{} & 
&
\multicolumn{1}{|l|}{{\sc Random}} &
\multicolumn{1}{c|}{${\bf0.47} (\pm 0.08)$} & \multicolumn{1}{c|}{${\bf5.81} (\pm 0.38)$} & \multicolumn{1}{c|}{$0.81 (\pm 0.05)$} & \multicolumn{1}{c|}{$4.59 (\pm 0.33)$}&
\multicolumn{1}{l|}{$0.12 (\pm 0.02)$} & \multicolumn{1}{c|}{$7.52 (\pm 0.47)$} & \multicolumn{1}{c|}{$0.23 (\pm 0.03)$} &
\multicolumn{1}{c|}{$5.17 (\pm 1.09)$} &
\multicolumn{1}{c|}{$0.09 (\pm 0.02)$} & \multicolumn{1}{c|}{$8.19 (\pm 0.21)$} & \multicolumn{1}{c|}{$0.10 (\pm 0.03)$} & \multicolumn{1}{c|}{$0.63 (\pm 1.60)$} 
\\
\cline{2-15}
\multicolumn{1}{|l|}{} & 
\multicolumn{1}{l}{\multirow{4}{*}{GCMC}} & 
\multicolumn{1}{|l|}{GREASE} &
\multicolumn{1}{l|}{$0.57 (\pm 0.06)$} & \multicolumn{1}{c|}{$6.33 (\pm 0.32)$} & \multicolumn{1}{c|}{$0.88 (\pm 0.08)$} &
\multicolumn{1}{c|}{$4.77 (\pm 0.53)$} &
\multicolumn{1}{l|}{$0.69 (\pm 0.08)$} & \multicolumn{1}{c|}{$8.42 (\pm 0.61)$} & \multicolumn{1}{c|}{$0.86 (\pm 0.08)$} &
\multicolumn{1}{c|}{$7.63 (\pm 1.09)$} &
\multicolumn{1}{c|}{$0.53 (\pm 0.06)$} & \multicolumn{1}{c|}{${\bf5.36}(\pm 0.42)$} & \multicolumn{1}{c|}{${\bf0.83} (\pm 0.03)$} & \multicolumn{1}{c|}{${\bf5.23} (\pm 0.42)$}
\\
\cline{3-15}
\multicolumn{1}{|l|}{} &
% \multicolumn{1}{l|}{GCMC} &
&
\multicolumn{1}{|l|}{{\sc PGExplainer}} &
\multicolumn{1}{l|}{$0.53 (\pm 0.05)$} & \multicolumn{1}{c|}{$6.66 (\pm 0.35)$} & \multicolumn{1}{c|}{$0.85 (\pm 0.06)$} &
\multicolumn{1}{c|}{$5.08 (\pm 0.53)$} &
\multicolumn{1}{l|}{$0.68 (\pm 0.07)$} & \multicolumn{1}{c|}{$8.49 (\pm 0.59)$} & \multicolumn{1}{c|}{$0.85 (\pm 0.08)$} &
\multicolumn{1}{c|}{$8.19 (\pm 0.98)$} &
\multicolumn{1}{c|}{$0.52 (\pm 0.03)$} &
\multicolumn{1}{c|}{$6.78 (\pm 0.47)$} & 
\multicolumn{1}{c|}{$0.79 (\pm 0.05)$} & 
\multicolumn{1}{c|}{$5.38 (\pm 0.36)$}
\\
\cline{3-15}
\multicolumn{1}{|l|}{} &
% \multicolumn{1}{l|}{GCMC} &
&
\multicolumn{1}{|l|}{{\sc PersonalRank}} &
\multicolumn{1}{l|}{$0.52 (\pm 0.05)$} & \multicolumn{1}{c|}{$6.35 (\pm 0.37)$} & \multicolumn{1}{c|}{$0.83 (\pm 0.06)$} &
\multicolumn{1}{c|}{$4.96 (\pm 0.52)$} &
\multicolumn{1}{l|}{$0.67 (\pm 0.07)$} & \multicolumn{1}{c|}{$8.36 (\pm 0.65)$} & \multicolumn{1}{c|}{$0.83 (\pm 0.06)$} &
\multicolumn{1}{c|}{$8.23 (\pm 0.96)$} &
\multicolumn{1}{c|}{${\bf0.53} (\pm 0.05)$} & \multicolumn{1}{c|}{$6.93 (\pm 0.52)$} & \multicolumn{1}{c|}{$0.78 (\pm 0.06)$} & \multicolumn{1}{c|}{$7.45 (\pm 0.53)$}
\\
\cline{3-15}
\multicolumn{1}{|l|}{} &
% \multicolumn{1}{l|}{} & 
&
\multicolumn{1}{|l|}{{\sc Random}} &
\multicolumn{1}{l|}{$0.13 (\pm 0.03)$} & \multicolumn{1}{c|}{$8.47 (\pm 0.62)$} & \multicolumn{1}{c|}{$0.19 (\pm 0.03)$} &
\multicolumn{1}{c|}{$5.00 (\pm 1.20)$} &
\multicolumn{1}{l|}{$0.18 (\pm 0.04)$} & \multicolumn{1}{c|}{$7.68 (\pm 0.86)$} & \multicolumn{1}{c|}{$0.26 (\pm 0.03)$} &
\multicolumn{1}{c|}{$7.62 (\pm 1.20)$} &
\multicolumn{1}{c|}{$0.06 (\pm 0.02)$} & \multicolumn{1}{c|}{$9.20 (\pm 0.32)$} & \multicolumn{1}{c|}{$0.13 (\pm 0.02)$} & \multicolumn{1}{c|}{$6.93 (\pm 0.37)$}
\\
\hline
\hline
% Yelp
\multicolumn{1}{|l|}{\multirow{12}{*}{\em Yelp}} & 
\multicolumn{1}{l}{\multirow{4}{*}{LightGCN}} & 
\multicolumn{1}{|l|}{GREASE} &
\multicolumn{1}{l|}{$0.56 (\pm 0.04)$} & \multicolumn{1}{c|}{$6.77 (\pm 0.50)$} & \multicolumn{1}{c|}{$0.90 (\pm 0.08)$} &
\multicolumn{1}{c|}{$3.79 (\pm 0.46)$} &
\multicolumn{1}{l|}{$0.67 (\pm 0.05)$} & \multicolumn{1}{c|}{$6.42 (\pm 0.41)$} & \multicolumn{1}{c|}{$0.88 (\pm 0.06)$} &
\multicolumn{1}{c|}{$3.45 (\pm 0.35)$} &
\multicolumn{1}{c|}{$\mathbf{0.58} (\pm 0.04)$} & \multicolumn{1}{c|}{$\mathbf{6.99} (\pm 0.32)$} & \multicolumn{1}{c|}{$\mathbf{0.76} (\pm 0.04)$} & \multicolumn{1}{c|}{$\mathbf{4.28} (\pm 0.38)$}
\\
\cline{3-15}
\multicolumn{1}{|l|}{} & 
% \multicolumn{1}{l|}{LightGCN} & 
&
\multicolumn{1}{|l|}{{\sc PGExplainer}} &
\multicolumn{1}{l|}{$0.56 (\pm 0.03)$} & \multicolumn{1}{c|}{$7.01 (\pm 0.43)$} & \multicolumn{1}{c|}{$0.90 (\pm 0.05$} &
\multicolumn{1}{c|}{$3.92 (\pm 0.43)$} &
\multicolumn{1}{l|}{$0.65 (\pm 0.03)$} & \multicolumn{1}{c|}{$6.89 (\pm 0.47)$} & \multicolumn{1}{c|}{$0.88 (\pm 0.05)$} &
\multicolumn{1}{c|}{$4.21 (\pm 0.36)$} &
\multicolumn{1}{c|}{$0.55 (\pm 0.03)$} & \multicolumn{1}{c|}{$7.32 (\pm 0.33)$} & \multicolumn{1}{c|}{$0.73 (\pm 0.04)$} & \multicolumn{1}{c|}{$4.19 (\pm 0.29)$} 
\\
\cline{3-15}
\multicolumn{1}{|l|}{} & 
% \multicolumn{1}{l|}{LightGCN} & 
&
\multicolumn{1}{|l|}{{\sc PersonalRank}} &
\multicolumn{1}{l|}{$0.55 (\pm 0.05)$} & \multicolumn{1}{c|}{$6.96 (\pm 0.47)$} & \multicolumn{1}{c|}{$0.89 (\pm 0.04)$} &
\multicolumn{1}{c|}{$4.15 (\pm 0.42)$} &
\multicolumn{1}{l|}{$0.61 (\pm 0.03)$} & \multicolumn{1}{c|}{$6.93 (\pm 0.41)$} & \multicolumn{1}{c|}{$0.82 (\pm 0.04)$} &
\multicolumn{1}{c|}{$4.79 (\pm 0.36)$} &
\multicolumn{1}{c|}{$0.53 (\pm 0.03)$} & \multicolumn{1}{c|}{$7.52 (\pm 0.73)$} & \multicolumn{1}{c|}{$0.71 (\pm 0.05)$} & \multicolumn{1}{c|}{$5.63 (\pm 0.45)$} 
\\
\cline{3-15}
\multicolumn{1}{|l|}{} & 
%\multicolumn{1}{l|}{} & 
&
\multicolumn{1}{|l|}{{\sc Random}} &
\multicolumn{1}{l|}{$0.16 (\pm 0.04)$} & \multicolumn{1}{c|}{$8.72 (\pm 0.66)$} & \multicolumn{1}{c|}{$0.21 (\pm 0.02)$} &
\multicolumn{1}{c|}{$5.36 (\pm 0.69)$} &
\multicolumn{1}{l|}{$0.15 (\pm 0.03)$} & \multicolumn{1}{c|}{$7.35 (\pm 0.13)$} & \multicolumn{1}{c|}{$0.21 (\pm 0.05)$} &
\multicolumn{1}{c|}{$5.39 (\pm 1.32)$} &
\multicolumn{1}{c|}{$0.08 (\pm 0.02)$} & \multicolumn{1}{c|}{$8.02 (\pm 0.19)$} & \multicolumn{1}{c|}{$0.13 (\pm 0.01)$} & \multicolumn{1}{c|}{$5.46 (\pm 1.72)$} 
\\
\cline{2-15}
\multicolumn{1}{|l|}{} & 
\multicolumn{1}{l}{\multirow{4}{*}{NGCF}} & 
\multicolumn{1}{|l|}{GREASE} &
\multicolumn{1}{l|}{$0.66 (\pm 0.06)$} & \multicolumn{1}{c|}{$8.37 (\pm 0.51)$} & \multicolumn{1}{c|}{$0.87 (\pm 0.05)$} &
\multicolumn{1}{c|}{$7.35 (\pm 1.12)$} &
\multicolumn{1}{l|}{$0.69 (\pm 0.05)$} & \multicolumn{1}{c|}{$6.21 (\pm 0.82)$} & \multicolumn{1}{c|}{$0.91 (\pm 0.06)$} &
\multicolumn{1}{c|}{$5.28 (\pm 0.30)$} &
\multicolumn{1}{c|}{$0.53 (\pm 0.04)$} & \multicolumn{1}{c|}{$\mathbf{4.36} (\pm 0.37)$} & 
\multicolumn{1}{c|}{$\mathbf{0.76} (\pm 0.04)$} & 
\multicolumn{1}{c|}{$\mathbf{3.75} (\pm 0.37)$}
\\
\cline{3-15}
\multicolumn{1}{|l|}{} & 
%\multicolumn{1}{l|}{} & 
&
\multicolumn{1}{|l|}{{\sc PGExplainer}} & 
\multicolumn{1}{l|}{$0.64(\pm 0.05)$} & \multicolumn{1}{c|}{$8.85 (\pm 0.60)$} & \multicolumn{1}{c|}{$0.88 (\pm 0.06)$} &
\multicolumn{1}{c|}{$7.43 (\pm 0.88)$} &
\multicolumn{1}{l|}{$0.68 (\pm 0.03)$} & \multicolumn{1}{c|}{$6.86 (\pm 0.43)$} & \multicolumn{1}{c|}{$0.86 (\pm 0.05)$} &
\multicolumn{1}{c|}{$5.76 (\pm 0.29)$} &
\multicolumn{1}{c|}{$0.53 (\pm 0.03)$} & \multicolumn{1}{c|}{$6.26 (\pm 0.39)$} & \multicolumn{1}{c|}{$0.75 (\pm 0.03)$} & \multicolumn{1}{c|}{$4.59 (\pm 0.38)$}
\\
\cline{3-15}
\multicolumn{1}{|l|}{} & 
%\multicolumn{1}{l|}{} & 
&
\multicolumn{1}{|l|}{{\sc PersonalRank}} &
\multicolumn{1}{l|}{$0.58 (\pm 0.07)$} & \multicolumn{1}{c|}{$8.76 (\pm 0.65)$} & \multicolumn{1}{c|}{$0.85 (\pm 0.08)$} &
\multicolumn{1}{c|}{$8.21 (\pm 0.96)$} &
\multicolumn{1}{l|}{$0.59 (\pm 0.04)$} & \multicolumn{1}{c|}{$7.21 (\pm 0.38)$} & \multicolumn{1}{c|}{$0.83 (\pm 0.03)$} &
\multicolumn{1}{c|}{$6.22 (\pm 0.41)$} &
\multicolumn{1}{c|}{${\bf0.55} (\pm 0.04)$} & \multicolumn{1}{c|}{$6.93 (\pm 0.42)$} & \multicolumn{1}{c|}{$0.74 (\pm 0.05)$} & \multicolumn{1}{c|}{$5.83 (\pm 0.45)$} 
\\
\cline{3-15}
\multicolumn{1}{|l|}{} & 
%\multicolumn{1}{l|}{} & 
&
\multicolumn{1}{|l|}{{\sc Random}} & 
\multicolumn{1}{l|}{$0.18 (\pm 0.03)$} & \multicolumn{1}{c|}{$7.68 (\pm 0.86)$} & \multicolumn{1}{c|}{$0.25 (\pm 0.03)$} &
\multicolumn{1}{c|}{$7.32 (\pm 1.20)$} &
\multicolumn{1}{l|}{$0.15 (\pm 0.01)$} & \multicolumn{1}{c|}{$8.60 (\pm 0.46)$} & \multicolumn{1}{c|}{$0.22 (\pm 0.02)$} &
\multicolumn{1}{c|}{$8.20 (\pm 1.47)$} &
\multicolumn{1}{c|}{$0.06 (\pm 1.00)$} & \multicolumn{1}{c|}{$6.35 (\pm 1.53)$} & \multicolumn{1}{c|}{$0.13 (\pm 0.03)$} & \multicolumn{1}{c|}{$6.21 (\pm 1.70)$}
\\
\cline{2-15}
\multicolumn{1}{|l|}{} & 
\multicolumn{1}{l}{\multirow{4}{*}{GCMC}} & 
\multicolumn{1}{|l|}{GREASE} &
\multicolumn{1}{l|}{$0.63 (\pm 0.04)$} & \multicolumn{1}{c|}{$7.21 (\pm 0.63)$} & \multicolumn{1}{c|}{$0.86 (\pm 0.07)$} &
\multicolumn{1}{c|}{$4.26 (\pm 0.55)$} &
\multicolumn{1}{l|}{$0.63 (\pm 0.05)$} & \multicolumn{1}{c|}{$7.31 (\pm 0.63)$} & \multicolumn{1}{c|}{$0.86 (\pm 0.07)$} &
\multicolumn{1}{c|}{$4.76 (\pm 0.52)$} &
\multicolumn{1}{c|}{${\bf0.74} (\pm 0.04)$} & \multicolumn{1}{c|}{${\bf4.14} (\pm 0.37)$} & \multicolumn{1}{c|}{$0.70 (\pm 0.06)$} & \multicolumn{1}{c|}{${\bf4.23} (\pm 0.43)$}
\\
\cline{3-15}
\multicolumn{1}{|l|}{} &
%\multicolumn{1}{l|}{} & 
&
\multicolumn{1}{|l|}{{\sc PGExplainer}} &
\multicolumn{1}{l|}{$0.61 (\pm 0.03)$} & \multicolumn{1}{c|}{$8.09 (\pm 0.58)$} & \multicolumn{1}{c|}{$0.86 (\pm 0.05)$} &
\multicolumn{1}{c|}{$4.38 (\pm 0.53)$} &
\multicolumn{1}{l|}{$0.64 (\pm 0.03)$} & \multicolumn{1}{c|}{$7.82 (\pm 0.52)$} & \multicolumn{1}{c|}{$0.85 (\pm 0.06)$} &
\multicolumn{1}{c|}{$4.92 (\pm 0.49)$} &
\multicolumn{1}{c|}{$0.72 (\pm 0.03)$} &
\multicolumn{1}{c|}{$5.31 (\pm 0.37)$} & \multicolumn{1}{c|}{$0.71 (\pm 0.05)$} & \multicolumn{1}{c|}{$4.36 (\pm 0.32)$} 
\\
\cline{3-15}
\multicolumn{1}{|l|}{} &
%\multicolumn{1}{l|}{GCMC} & 
&
\multicolumn{1}{|l|}{{\sc PersonalRank}} &
\multicolumn{1}{l|}{$0.60 (\pm 0.04)$} & \multicolumn{1}{c|}{$8.16 (\pm 0.75)$} & \multicolumn{1}{c|}{$0.82 (\pm 0.05)$} &
\multicolumn{1}{c|}{$4.53 (\pm 0.61)$} &
\multicolumn{1}{l|}{$0.63 (\pm 0.05)$} & \multicolumn{1}{c|}{$7.98 (\pm 0.75)$} & \multicolumn{1}{c|}{$0.81 (\pm 0.06)$} &
\multicolumn{1}{c|}{$5.23 (\pm 0.61)$} &
\multicolumn{1}{c|}{$0.72 (\pm 0.05)$} & \multicolumn{1}{c|}{$5.63 (\pm 0.43)$} & \multicolumn{1}{c|}{${\bf0.71} (\pm 0.06)$} & \multicolumn{1}{c|}{$4.86 (\pm 0.51)$}
\\
\cline{3-15}
\multicolumn{1}{|l|}{} &
%\multicolumn{1}{l|}{} & 
&
\multicolumn{1}{|l|}{{\sc Random}} &
\multicolumn{1}{l|}{$0.12 (\pm 0.02)$} & \multicolumn{1}{c|}{$8.53 (\pm 0.66)$} & \multicolumn{1}{c|}{$0.17 (\pm 0.05)$} &
\multicolumn{1}{c|}{$8.31 (\pm 1.16)$} &
\multicolumn{1}{l|}{$0.15 (\pm 0.02)$} & \multicolumn{1}{c|}{$8.42 (\pm 0.57)$} & \multicolumn{1}{c|}{$0.16 (\pm 0.05)$} &
\multicolumn{1}{c|}{$8.37 (\pm 1.09)$} &
\multicolumn{1}{c|}{$0.10 (\pm 0.02)$} & \multicolumn{1}{c|}{$5.43 (\pm 0.23)$} & \multicolumn{1}{c|}{$0.13 (\pm 0.02)$} & \multicolumn{1}{c|}{$5.73 (\pm 0.17)$}
\\
\hline
\hline
% Gowalla
\multicolumn{1}{|l|}{\multirow{12}{*}{\em Gowalla}} & 
\multicolumn{1}{l}{\multirow{4}{*}{LightGCN}} & 
\multicolumn{1}{|l|}{GREASE} &
\multicolumn{1}{l|}{$0.72 (\pm 0.07)$} & \multicolumn{1}{c|}{$6.89 (\pm 0.42)$} & \multicolumn{1}{c|}{$0.92 (\pm 0.06)$} &
\multicolumn{1}{c|}{$4.89 (\pm 0.51)$} &
\multicolumn{1}{l|}{$0.85 (\pm 0.06)$} & \multicolumn{1}{c|}{$6.83 (\pm 0.42)$} & \multicolumn{1}{c|}{$0.95 (\pm 0.09)$} &
\multicolumn{1}{c|}{$6.21 (\pm 0.33)$} &
\multicolumn{1}{c|}{$0.45 (\pm 0.05)$} & \multicolumn{1}{c|}{$\mathbf{5.56} (\pm 0.27)$} & 
\multicolumn{1}{c|}{$\mathbf{0.83} (\pm 0.08)$} & 
\multicolumn{1}{c|}{ $\mathbf{3.75} (\pm 0.37)$}
\\
\cline{3-15}
\multicolumn{1}{|l|}{} & 
%\multicolumn{1}{l|}{} & 
&
\multicolumn{1}{|l|}{{\sc PGExplainer}} & 
\multicolumn{1}{l|}{$0.72 (\pm 0.05)$} & \multicolumn{1}{c|}{$7.02 (\pm 0.36)$} & \multicolumn{1}{c|}{$0.88 (\pm 0.04)$} &
\multicolumn{1}{c|}{$4.96 (\pm 0.47)$} &
\multicolumn{1}{l|}{$0.83 (\pm 0.05)$} & \multicolumn{1}{c|}{$7.18 (\pm 0.36)$} & \multicolumn{1}{c|}{$0.93 (\pm 0.07)$} &
\multicolumn{1}{c|}{$6.38 (\pm 0.28)$} & \multicolumn{1}{c|}{$0.43 (\pm 0.04)$} & \multicolumn{1}{c|}{$5.92 (\pm 0.31)$} &
\multicolumn{1}{c|}{$0.80 (\pm 0.05)$} & \multicolumn{1}{c|}{$4.06 (\pm 0.30)$} 
\\
\cline{3-15}
\multicolumn{1}{|l|}{} & 
%\multicolumn{1}{l|}{LightGCN} & 
&
\multicolumn{1}{|l|}{{\sc PersonalRank}} & 
\multicolumn{1}{l|}{$0.72 (\pm 0.06)$} & \multicolumn{1}{c|}{$6.95 (\pm 0.39)$} & \multicolumn{1}{c|}{$0.89(\pm 0.05)$} &
\multicolumn{1}{c|}{$4.79 (\pm 0.56)$} &
\multicolumn{1}{l|}{$0.77 (\pm 0.08)$} & \multicolumn{1}{c|}{$7.23 (\pm 0.47)$} & \multicolumn{1}{c|}{$0.93 (\pm 0.12)$} &
\multicolumn{1}{c|}{$6.32 (\pm 0.31)$} &
\multicolumn{1}{c|}{${\bf0.45} (\pm 0.06)$} & \multicolumn{1}{c|}{$5.88 (\pm 0.31)$} & \multicolumn{1}{c|}{$0.81 (\pm 0.06)$} & \multicolumn{1}{c|}{$4.13 (\pm 0.32)$} 
\\
\cline{3-15}
\multicolumn{1}{|l|}{} & 
%\multicolumn{1}{l|}{} & 
&
\multicolumn{1}{|l|}{{\sc Random}} & 
\multicolumn{1}{l|}{$0.13 (\pm 0.04)$} & \multicolumn{1}{c|}{$8.15 (\pm 1.32)$} & \multicolumn{1}{c|}{$0.27 (\pm 0.05)$} &
\multicolumn{1}{c|}{$7.39 (\pm 1.16)$} &
\multicolumn{1}{l|}{$0.18 (\pm 0.05)$} & \multicolumn{1}{c|}{$7.36 (\pm 0.99)$} & \multicolumn{1}{c|}{$0.27 (\pm 0.09)$} &
\multicolumn{1}{c|}{$7.02 (\pm 1.05)$} &
\multicolumn{1}{c|}{$0.05 (\pm 0.02)$} & \multicolumn{1}{c|}{$6.73 (\pm 0.36)$} & \multicolumn{1}{c|}{$0.16 (\pm 0.01)$} & \multicolumn{1}{c|}{$6.33 (\pm 0.10)$} 
\\
\cline{2-15}
\multicolumn{1}{|l|}{} & 
\multicolumn{1}{l}{\multirow{4}{*}{NGCF}} & 
\multicolumn{1}{|l|}{GREASE} &
\multicolumn{1}{l|}{$0.65 (\pm 0.05)$} & \multicolumn{1}{c|}{$6.43 (\pm 0.72)$} & \multicolumn{1}{c|}{$0.93 (\pm 0.09)$} &
\multicolumn{1}{c|}{$4.89 (\pm 0.51)$} &
\multicolumn{1}{l|}{$0.81 (\pm 0.06)$} & \multicolumn{1}{c|}{$7.23 (\pm 0.36)$} & \multicolumn{1}{c|}{$0.97 (\pm 0.04)$} &
\multicolumn{1}{c|}{$6.31 (\pm 0.29)$} &
\multicolumn{1}{c|}{$0.50 (\pm 0.09)$} & \multicolumn{1}{c|}{$5.32 (\pm 0.39)$} & \multicolumn{1}{c|}{$\mathbf{0.85} (\pm 0.06)$} & 
\multicolumn{1}{c|}{$\mathbf{4.23} (\pm 0.22)$}
\\
\cline{3-15}
\multicolumn{1}{|l|}{} & 
%\multicolumn{1}{l|}{} & 
&
\multicolumn{1}{|l|}{{\sc PGExplainer}} & 
\multicolumn{1}{l|}{$0.65 (\pm 0.03)$} & \multicolumn{1}{c|}{$7.08 (\pm 0.46)$} & \multicolumn{1}{c|}{$0.94 (\pm 0.08)$} &
\multicolumn{1}{c|}{$5.03 (\pm 0.43)$} &
\multicolumn{1}{l|}{$0.81 (\pm 0.03)$} & \multicolumn{1}{c|}{$7.56 (\pm 0.27)$} & \multicolumn{1}{c|}{$0.96 (\pm 0.04)$} &
\multicolumn{1}{c|}{$6.39 (\pm 0.31)$} &
\multicolumn{1}{c|}{$0.49 (\pm 0.07)$} & \multicolumn{1}{c|}{$5.39 (\pm 0.36)$} & \multicolumn{1}{c|}{$0.83 (\pm 0.04)$} & \multicolumn{1}{c|}{$4.49 (\pm 0.22)$} 
\\
\cline{3-15}
\multicolumn{1}{|l|}{} & 
%\multicolumn{1}{l|}{} & 
&
\multicolumn{1}{|l|}{{\sc PersonalRank}} & 
\multicolumn{1}{l|}{$0.65 (\pm 0.07)$} & \multicolumn{1}{c|}{$7.23 (\pm 0.58)$} & \multicolumn{1}{c|}{$0.92 (\pm 0.08)$} &
\multicolumn{1}{c|}{$6.22 (\pm 0.52)$} &
\multicolumn{1}{l|}{$0.79 (\pm 0.09)$} & \multicolumn{1}{c|}{$7,65 (\pm 0.43)$} & \multicolumn{1}{c|}{$0.96 (\pm 0.08)$} &
\multicolumn{1}{c|}{$6.42 (\pm 0.34)$} &
\multicolumn{1}{c|}{${\bf0.51} (\pm 0.08)$} & \multicolumn{1}{c|}{${\bf5.27} (\pm 0.52)$} & \multicolumn{1}{c|}{${\bf0.85} (\pm 0.04)$} & \multicolumn{1}{c|}{$4.39 (\pm 0.26)$} 
\\
\cline{3-15}
\multicolumn{1}{|l|}{} & 
%\multicolumn{1}{l|}{} & 
&
\multicolumn{1}{|l|}{{\sc Random}} & 
\multicolumn{1}{l|}{$0.15 (\pm 0.06)$} & \multicolumn{1}{c|}{$8.60 (\pm 0.53)$} & \multicolumn{1}{c|}{$0.22 (\pm 0.03)$} &
\multicolumn{1}{c|}{$8.20 (\pm 1.47)$} &
\multicolumn{1}{l|}{$0.13 (\pm 0.05)$} & \multicolumn{1}{c|}{$8.37 (\pm 0.49)$} & \multicolumn{1}{c|}{$0.19 (\pm 0.05)$} &
\multicolumn{1}{c|}{$8.15 (\pm 0.77)$} &
\multicolumn{1}{c|}{$0.09 (\pm 0.03)$} & \multicolumn{1}{c|}{$6.32 (\pm 0.45)$} & \multicolumn{1}{c|}{$0.21 (\pm 0.02)$} & \multicolumn{1}{c|}{$5.57 (\pm 0.16)$}
\\
\cline{2-15}
\multicolumn{1}{|l|}{} &
\multicolumn{1}{l}{\multirow{4}{*}{GCMC}} & 
\multicolumn{1}{|l|}{GREASE} &
\multicolumn{1}{l|}{$0.58 (\pm 0.05)$} & \multicolumn{1}{c|}{$8.43 (\pm 0.52)$} & \multicolumn{1}{c|}{$0.87 (\pm 0.08)$} &
\multicolumn{1}{c|}{$7.68 (\pm 0.97)$} &
\multicolumn{1}{l|}{$0.60 (\pm 0.06)$} & \multicolumn{1}{c|}{$8.75 (\pm 0.53)$} & \multicolumn{1}{c|}{$0.88 (\pm 0.09)$} &
\multicolumn{1}{c|}{$7.75 (\pm 1.05)$} &
\multicolumn{1}{c|}{$0.46 (\pm 0.09)$} & \multicolumn{1}{c|}{$5.85 (\pm 0.33)$} & \multicolumn{1}{c|}{${\bf0.82} (\pm 0.04)$} & \multicolumn{1}{c|}{${\bf4.32} (\pm 0.29)$}
\\
\cline{3-15}
\multicolumn{1}{|l|}{} &
%\multicolumn{1}{l|}{} & 
&
\multicolumn{1}{|l|}{{\sc PGExplainer}} &
\multicolumn{1}{l|}{$0.59 (\pm 0.06)$} & \multicolumn{1}{c|}{$8.68 (\pm 0.45)$} & \multicolumn{1}{c|}{$0.86 (\pm 0.07)$} &
\multicolumn{1}{c|}{$8.16 (\pm 0.86)$} &
\multicolumn{1}{l|}{$0.58 (\pm 0.07)$} & \multicolumn{1}{c|}{$8.56 (\pm 0.48)$} & \multicolumn{1}{c|}{$0.86 (\pm 0.05)$} &
\multicolumn{1}{c|}{$8.15 (\pm 0.83)$} &
\multicolumn{1}{c|}{$0.45 (\pm 0.07)$} & \multicolumn{1}{c|}{$5.93 (\pm 0.31)$} & \multicolumn{1}{c|}{$0.81 (\pm 0.04)$} & \multicolumn{1}{c|}{$4.27 (\pm 0.26)$}
\\
\cline{3-15}
\multicolumn{1}{|l|}{} &
%\multicolumn{1}{l|}{} & 
&
\multicolumn{1}{|l|}{{\sc PersonalRank}} &
\multicolumn{1}{l|}{$0.58 (\pm 0.07)$} & \multicolumn{1}{c|}{$8.76 (\pm 0.65)$} & \multicolumn{1}{c|}{$0.85 (\pm 0.06)$} &
\multicolumn{1}{c|}{$8.21 (\pm 0.96)$} &
\multicolumn{1}{l|}{$0.61 (\pm 0.07)$} & \multicolumn{1}{c|}{$8.83 (\pm 0.65)$} & \multicolumn{1}{c|}{$0.85 (\pm 0.06)$} &
\multicolumn{1}{c|}{$8.32 (\pm 0.88)$} &
\multicolumn{1}{c|}{${\bf0.47} (\pm 0.08)$} & \multicolumn{1}{c|}{${\bf5.81} (\pm 0.38)$} & \multicolumn{1}{c|}{$0.81 (\pm 0.05)$} & \multicolumn{1}{c|}{$4.59 (\pm 0.33)$}
\\
\cline{3-15}
\multicolumn{1}{|l|}{} &
%\multicolumn{1}{l|}{} & 
&
\multicolumn{1}{|l|}{{\sc Random}} &
\multicolumn{1}{l|}{$0.18 (\pm 0.04)$} & \multicolumn{1}{c|}{$7.68 (\pm 0.86)$} & \multicolumn{1}{c|}{$0.25 (\pm 0.03)$} &
\multicolumn{1}{c|}{$7.32 (\pm 1.20)$} &
\multicolumn{1}{l|}{$0.20 (\pm 0.04)$} & \multicolumn{1}{c|}{$7.38 (\pm 0.86)$} & \multicolumn{1}{c|}{$0.28 (\pm 0.03)$} &
\multicolumn{1}{c|}{$7.28 (\pm 1.20)$} &
\multicolumn{1}{c|}{$0.06 (\pm 0.01)$} & \multicolumn{1}{c|}{$8.23 (\pm 0.57)$} & \multicolumn{1}{c|}{$0.16 (\pm 0.03)$} & \multicolumn{1}{c|}{$5.00 (\pm 0.96)$}
\\
\hline
\end{tabular}
}
\caption{\label{tab:all-results}
PS($\uparrow$), PN($\uparrow$), and EC($\downarrow$) of factual and counterfactual explanations generated by \textsc{\textbf{GREASE}}, \textsc{\textbf{PGExplainer}}, \textsc{\textbf{PersonalRank}}, and \textsc{\textbf{Random}} for top-$10$, top-$15$, and top-$20$ recommended items according to LightGCN, NGCF, and GCMC GNN-based recommender systems trained on \textit{LastFM}, \textit{Yelp}, and \textit{Gowalla} datasets.}
%\vspace{-3mm}
\end{table*}

==> theory.tex <==
\section{Theoretical Analysis}
\label{sec:Theory}
We provide a theoretical analysis of CURE to indicate that a single gradient update on the model parameters of CURE achieves lower loss than normal gradient descent. Let $\Theta=\{\orishare, \oriforget, \oriretain\}$ denote the parameters of components in selected circuits. After applying CURE, the model parameters are $\hat{\Theta}=\{\selshare,\selforget, \selretain \}$. An one step gradient update of $\hat{\Theta}$ is:
\begin{equation}
\label{eq:CUREupdate}
\begin{aligned}
\hat{\theta}_{sh}
&= \theta_{sh}
- \alpha\Big[
\wretain \Big(
\gradrshare
- \frac{\gradrshare \cdot \gradfshare}{\|\gradfshare\|^2}\,\gradfshare
\Big)
+ \wforget \Big(
\gradfshare
- \frac{\gradfshare \cdot \gradrshare}{\|\gradrshare\|^2}\,\gradrshare
\Big)
\Big], \\
\hat{\theta}_f &= \theta_f - \alpha\gradfforget,
\qquad
\hat{\theta}_r = \theta_r - \alpha\gradrretain .
\end{aligned}
\end{equation}
Without applying CURE, the parameters are
$\Tilde{\Theta}=\{\nshare\,\nforget, \nretain\}$. An one-step gradient update is given by:
\begin{equation}
\label{eq:SGDupdate}
\begin{aligned}
\tilde{\theta}_i &= \theta_i - \alpha(\wretain \mathbf{g}_{i}^{R} + \wforget \mathbf{g}_{i}^{F}), \quad i \in \{sh, f, r\}
\end{aligned}
\end{equation}
Then, we have the following theorem. 
\begin{theorem}
Assume that the joint loss function is defined as
$L(\Theta) = \wretain L_R(\Theta) + \wforget L_F(\Theta)$ and $\wretain+\wforget=1$. Then for any sufficiently small learning rate $\alpha>0$, we have
\begin{equation}
\label{eq:Objective}
\begin{aligned}
L(\hat{\Theta})\leq L(\Tilde{\Theta})
\end{aligned}
\end{equation}
\end{theorem}

% \textbf{Proof Sketch.}

% By applying the first order Taylor approximation of L, we have

% \begin{equation}
% \label{eq:Taylor Expansion}
% \begin{aligned}
% L(\Tilde{\Theta})&=L_{f}(\nshare,\nforget)+L_{r}(\nshare,\nretain)\\
% &=L(\orishare)+(\nshare-\orishare)(\gradfshare+\gradrshare)\\
% &+(\nforget-\oriforget)\gradfforget+(\nretain-\oriretain)\gradrretain+O(\alpha) \\
% L(\Hat{\Theta})&=L_{f}(\selshare,\selforget)+L_{r}(\selshare,\selretain)\\
% &=L(\orishare)+(\nshare-\orishare)(\gradfshare+\gradrshare)\\
% &+(\selforget-\oriforget)\gradfforget+(\selretain-\oriretain)\gradrretain+O(\alpha)
% \end{aligned}
% \end{equation}
% We have:

% \begin{equation}
% \label{eq:Substration}
% \begin{aligned}
% L(\Tilde{\Theta})-
% L(\Hat{\Theta})&=(\nforget-\selforget)\gradfforget+(\nretain-\selretain)\gradrretain \\
% &=\alpha(\wretain(\gradfforget-\gradrforget)\gradfforget+\wforget(\gradrretain-\gradfretain)\gradrretain)\\
% &=\alpha(\wretain(||\gradfforget||^2-{\gradrforget}^{\mbox{T}}\gradfforget)+\wforget(||\gradrretain||^2-{\gradfretain}^{\mbox{T}}\gradrretain))
% \end{aligned}
% \end{equation}

% Due to the greedy selection policy of neuron, we have 

% \begin{equation}
% \label{eq:Greedy}
% \begin{aligned}
% ||\mathbf{u^{1}}\gradfforget||^2\geq ||\mathbf{u^{1}}\gradrforget||^2, ||\mathbf{u^{2}}\gradrretain||^2\geq ||\mathbf{u^{1}}\gradfretain||^2
% \end{aligned}
% \end{equation}
% Where $\mathbf{u^{1}}$ and $\mathbf{u^{2}}$ are activation functions. Then we have


% \begin{equation}
% \label{eq:Greedy}
% \begin{aligned}
% 2||\mathbf{u^{1}}\gradfforget||^2\geq ||\mathbf{u^{1}}\gradrforget||^2+||\mathbf{u^{1}}\gradfforget||^2\geq ||\mathbf{u^{1}}||^2{\gradrforget}^{\mbox{T}}\gradfforget
% \end{aligned}
% \end{equation}

% Hence we have 
% \[L(\Tilde{\Theta})-
% L(\Hat{\Theta}) \geq 0\]



% % start proof
% $\params = \{ \orishare, \oriforget, \oriretain \}$



% $\params = \{ \orishare, \oriforget, \oriretain \}$

% \noindent\textbf{Update Rule.}
% \begin{align}
%     \text{Old: } \tilde{\theta}_i &= \theta_i - (w_r \mathbf{g}_{i}^{R} + w_f \mathbf{g}_{i}^{F}), \quad i \in \{sh, f, r\} \\[4pt]
%     \text{CURE: } \hat{\theta}_{sh} &= \theta_{sh} - \Big[ w_r \left( \gradrshare - \frac{\gradrshare \cdot \gradfshare}{\|\gradfshare\|^2} \gradfshare \right) \nonumber \\
%     &\quad + w_f \left( \gradfshare - \frac{\gradfshare \cdot \gradrshare}{\|\gradrshare\|^2} \gradrshare \right) \Big] \\
%     \hat{\theta}_f &= \theta_f - \gradfforget \\
%     \hat{\theta}_r &= \theta_r - \gradrretain
% \end{align}


% \begin{equation}
% \begin{aligned}
%     &\Loss(\tilde{\params}) - \Loss(\hat{\params}) \approx (\nshare - \selshare)^\top (\gradrshare + \gradfshare) + (\nforget - \selforget)^\top \gradfforget + (\nretain - \selretain)^\top \gradrretain \\
%     &\approx -\left[ \wretain \left( \frac{(\gradrshare \cdot \gradfshare)^2}{\|\gradfshare\|^2} + \gradrshare \cdot \gradfshare \right) + \wforget \left( \gradrshare \cdot \gradfshare + \frac{(\gradfshare \cdot \gradrshare)^2}{\|\gradrshare\|^2} \right) \right] \\
%     &= -\left[ (\gradrshare \cdot \gradfshare) + \wretain \frac{(\gradrshare \cdot \gradfshare)^2}{\|\gradfshare\|^2} + \wforget \frac{(\gradrshare \cdot \gradfshare)^2}{\|\gradrshare\|^2} \right]
% \end{aligned}
% \end{equation}

% To ensure that CURE outperforms the conventional update (i.e., $\Loss(\tilde{\params}) > \Loss(\hat{\params})$), the following condition must be satisfied:
% \begin{equation}
%     -(\gradrshare \cdot \gradfshare) > \wretain \frac{(\gradrshare \cdot \gradfshare)^2}{\|\gradfshare\|^2} + \wforget \frac{(\gradrshare \cdot \gradfshare)^2}{\|\gradrshare\|^2}
% \end{equation}

% By substituting $\gradrshare \cdot \gradfshare = \|\gradrshare\|\|\gradfshare\|\cos \theta$ and defining $\gamma = \frac{\|\gradrshare\|}{\|\gradfshare\|}$, we obtain the convergence condition:
% \begin{equation}
%     \cos \theta > -\frac{\gamma}{\wretain \gamma^2 + (1 - \wretain)}, \quad \text{where } \gamma = \frac{\|\gradrshare\|}{\|\gradfshare\|}
% \end{equation}


\noindent\textbf{Proof.} We iteratively update each parameter group while fixing the others. The loss difference between the conventional update $\tilde{\params}$ and CURE $\hat{\params}$ is analyzed via two components, $A$ and $B$:
\begin{equation}
\begin{aligned}
    &\Loss(\Tilde{\Theta}) - \Loss(\hat{\Theta}) \approx (\nshare - \selshare)^\top (\gradrshare + \gradfshare) \\
    &\quad + (\nforget - \selforget)^\top \gradfforget + (\nretain - \selretain)^\top \gradrretain \\
    &= \underbrace{-\Big[ \gradrshare \cdot \gradfshare + (\gradrshare \cdot \gradfshare)^2 \big( \tfrac{\wretain}{\|\gradfshare\|^2} + \tfrac{\wforget}{\|\gradrshare\|^2} \big) \Big]}_{A} \\
    &\quad + \underbrace{\wretain(\gradfforget - \gradrforget)^\top \gradfforget + \wforget(\gradrretain - \gradfretain)^\top \gradrretain}_{B}
\end{aligned}
\end{equation}

\noindent\textbf{For Part A:}
Let $\gamma = \|\gradrshare\| / \|\gradfshare\|$ and $\psi$ be the angle between $\gradrshare$ and $\gradfshare$.
% Part $A$ can be expanded and simplified as:
% \begin{equation}
% \begin{aligned}
%     A = - \Big[ \gradrshare \cdot \gradfshare + (\gradrshare \cdot \gradfshare)^2 \big( \tfrac{\wretain}{\|\gradfshare\|^2} + \tfrac{\wforget}{\|\gradrshare\|^2} \big) \Big]
% \end{aligned}
% \end{equation}
$A \ge 0$ is guaranteed if and only if the condition holds:
\begin{equation}
\label{equ:Acondition}
    \cos \psi \ge -\frac{\gamma}{\wretain + (1 - \wretain)\gamma^2}
\end{equation}
When $\gamma$ is close to $1$, indicating that the two gradients have comparable magnitudes, equation~\ref{equ:Acondition} holds with high probability.
Notably, when $\gamma = 1$, the condition reduces to $\cos \psi \ge -1$, which is \emph{always satisfied}.
In practice, we control $\gamma$ through gradient normalization, ensuring that the magnitudes of the two gradients remain comparable.

\noindent\textbf{For Part B:} We consider neurons in each task-specific component, and denote $\Delta m=(m^{*}_{v_1\to v_2}-m_{v_1\to v_2})$ in equation~\ref{eq:ActivationPatching}.
According to the loss functions $\mathcal{L}_{F}$ and $\mathcal{L}_{R}$ defined in Section~\ref{sec:selupdate}, we observe that both losses are monotonic with respect to
$\Delta(\inpori)=\LLMori(Yes|\inpori)-\LLMori(No|\inpori)$, which is used to detected the forget and retain circuits. which is used to detect forget and retain circuits. Hence, the greedy selection policy in Section~\ref{sec:greedy} satisfies:
\begin{equation}
\begin{aligned}
    & \|\Delta m \gradfforget\|^2 \ge \|\Delta m \gradrforget\|^2, \quad \|\Delta m \gradrretain\|^2 \ge \|\Delta m \gradfretain\|^2 \\
    & \implies 2\|\Delta m \gradfforget\|^2 \ge \|\Delta m \gradfforget\|^2 + \|\Delta m \gradrforget\|^2 \\
    & \quad \ge \|\Delta m\|^2 (\gradfforget \cdot \gradrforget) \implies \|\gradfforget\|^2 - \gradfforget \cdot \gradrforget \ge 0
\end{aligned}
\end{equation}
This leads to $\|\gradfforget\|^2 - \gradfforget \cdot \gradrforget > 0$, ensuring the benefit of targeted forgetting. An analogous result can be derived $\|\gradrretain\|^2 - \gradfretain \cdot \gradrretain > 0$
